Grammar-Based Graph Compression

We present a new graph compressor that works by recursively detecting repeated substructures and representing them through grammar rules. We show that for a large number of graphs the compressor obtains smaller representations than other approaches. Specific queries such as reachability between two nodes or regular path queries can be evaluated in linear time (or quadratic times, respectively), over the grammar, thus allowing speed-ups proportional to the compression ratio.

==> introduction.tex <==
\section{Introduction}
Large graphs have been gaining importance over the past years: 
be it RDF graphs and the semantic web or social networks such as Facebook.
There is a plethora of recent research papers dealing with the analysis 
of large graphs, see e.g.,~\cite{DBLP:conf/sigmod/FanWW14,
%DBLP:conf/sigmod/SatishSPSPHSYD14,
DBLP:conf/sigmod/HanLL13,
%DBLP:conf/sigmod/ShaoWX12,
DBLP:conf/icde/CaoFHH15,
DBLP:conf/icde/WangXSW14%
%DBLP:conf/icde/SeoGL13
}.
Naturally, compression is an important technique for dealing with large
graphs, cf. Fan~\cite{DBLP:conf/icdt/Fan12}.
It can be applied in many different ways. 
For instance, systems that use distributed processing (e.g., via Map/Reduce) need to
repeatedly send large graphs over the network. Sending these graphs in a compressed
form can have a huge impact on the performance of the whole system; 
see e.g., the Pegasus system~\cite{DBLP:journals/kais/KangTF11}, 
which applies off-the-shelf gzip compression to an appropriately
permuted matrix representation of the graph~\cite{DBLP:conf/icassp/KangCF12}. Other applications are
to use the compressed graph as in-memory representation, or, to build from it specialized indexes
that support certain queries. An example for the first application is the compressed RDF graph
representation by \'Alvarez-Garc\'ia et al.~\cite{DBLP:journals/kais/Alvarez-GarciaB15}, an example for
the second is the query-based compression by Fan et al.~\cite{DBLP:conf/sigmod/FanLWW12} which removes
substructures from the graph that are not relevant for the supported class of queries.

Outside of the database community, compression of large network graphs has been studied already for
more than a decade,  possibly starting with the WebGraph framework by Boldi and
Vigna~\cite{DBLP:conf/www/BoldiV04}. Their methods proved very effective in compressing web graphs,
but are less effective for other graphs, such as social
graphs~\cite{DBLP:conf/kdd/ChierichettiKLMPR09}. Furthermore, network graphs are
commonly unlabeled and their methods are thus difficult to adapt to graphs with data, such as
RDF graphs.

Grammar-based compression is an attractive formalism of compression. The idea is to represent
data by a context-free grammar. Consider the string \textit{ababab}. It can be
represented by the grammar $\{ S\to AAA, A\to ab\}$,
%\[
%    \begin{array}{lcl}
%        S&\to& AAA\\
%        A&\to& ab
%    \end{array}
%\]
whose size (sum of lengths of right-hand sides) is smaller than the given string. Remarkably, this
simple formalism can be used to capture %LZ1-variant~\cite{DBLP:conf/stoc/FarachT95} of the
well-known compression schemes, such as Lempel-Ziv, see~\cite{Charikar05_smallest}. 
The attractiveness of grammar-based compression stems from its simplicity
and mathematical elegance. It can, for instance, be used to explain one of the first grep-algorithms
for compressed strings~\cite{DBLP:journals/jcss/AmirBF96}. Besides grep there are many problems that
can be solved in one pass through the grammar (see~\cite{Lohrey12_stringSLPsurvey}), thus providing a
\emph{speed-up} that is proportional to the compression ratio.
How can we find a smallest grammar for a given string? This problem is
\NP-complete~\cite{Charikar05_smallest}. Various approximation algorithms have been
proposed, one of which is the RePair compression scheme invented by
Larsson and Moffat~\cite{Larsson00_rePair}. It is a linear-time
approximation algorithm that compresses well in practice.
RePair was generalized to trees by Lohrey at al.~\cite{Lohrey13_treeRePair}.
Grammar-based compression typically produces two parts: a set of rules and an (often large)
incompressible, remaining part. 
%Figure~\ref{fig:graph} shows a graph on the left and its incompressible part,
%with respect to our new graph compressor.
%it's remaining structure on the right. We store this remaining
%graph using the \ktree data structure~\cite{Brisaboa09_k2Trees} and mainly compare against the
%uncompressed use of this data structure.
%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.45\linewidth]{figures/before.pdf}
%    \includegraphics[width=0.45\linewidth]{figures/after.pdf}
%    \caption{A DBLP version graph and its incompressible subgraph. 
%Here, 19\% of the 
%    nodes and 37\% of the edges remain in the incompressible subgraph.}
%    \label{fig:graph}
%\end{figure}
%\begin{figure*}[!t]
%    \centering
%    \subfloat[]{\input{figures/counting_example_center}\label{fig:counting_example_center}}\qquad
%    \subfloat[]{\input{figures/counting_example_dfs}\label{fig:counting_example_dfs}}\qquad
%    \subfloat[]{\input{figures/counting_example_opt}\label{fig:counting_example_opt}}\qquad
%    \subfloat[]{\input{figures/counting_example_digram}\label{fig:counting_example_digram}}
%    \caption{Three different traversals lead to three different frequency counts.}
%    \label{fig:counting_example}
%\end{figure*}
%\begin{figure}[!t]
%    \centering
%    \input{figures/grammar_example}
%    \caption{Example of a hyperedge replacement grammar.}
%    \label{fig:grammar_example}
%\end{figure}

We propose a generalization of RePair compression to graphs,
to be precise, to directed edge-labeled hypergraphs. 
The idea of RePair is to repeatedly replace a most frequent digram (in a string, a digram
is a pair of adjacent letters) by a new nonterminal, until no digram occurs more than once. 
In our setting, a digram consists of a pair of connected hyperedges. Let us consider an example:
Figure~\ref{fig:intro_grammar_example} shows a grammar with initial graph $S$, and one nonterminal
$A$, appearing three times in $S$. The rule for $A$ generates a digram -- two connected edges.
%
We apply the rule by removing an $A$-edge, and inserting the digram, so that source and target nodes
of the removed edge are merged with the source and target nodes of the digram. By applying the $A$-rule
three times to the start graph, we obtain the terminal graph, which consists of three $a$- and
$b$-edges as shown in Figure~\ref{fig:intro_derivation_example}.
%
%When
%applying the rule, its right-hand side is inserted into the graph by
%merging its \emph{source}-node (\emph{target}-node) with the source (target) of the nonterminal edge. The
%full step-by-step derivation of this grammar is given in Figure~\ref{fig:intro_derivation_example}.
%Thus, every rule has nodes, that are solely used to be merged with the nodes incident to the
%nonterminal. These nodes are called \emph{external} and are generally colored (in this case black).
%
RePair compression intuitively does the reverse of the rule-application shown in
Figure~\ref{fig:intro_derivation_example}. Starting with the full
graph, it replaces edge pairs that occur more than once by nonterminal edges, and introduces
corresponding rules. Thus it finds the digram consisting of an $a$- and a $b$-edge three times, and
replaces each by an $A$-edge (introducing the $A$-rule).
%
In general, the right-hand side of a rule can have several source and target nodes and we just speak
of ``external'' nodes (e.g. the black nodes in Figure~\ref{fig:intro_grammar_example}). A rule with
$k$ external nodes is applied to a \emph{hyperedge} with $k$ incident nodes. It is well-known that
restricting to rules (and start graph) with at most $k$ nodes generates (hyper)graphs of
tree-width at most $k$. The need to introduce hyperedges and right-hand sides with more than two
external nodes can be outlined on a slight modification of the graph in
Figure~\ref{fig:intro_derivation_example}, shown in Figure~\ref{fig:intro_rank3_example}. It has two
additional $c$-edges. The most frequent digram is still the one with one $a$- and one
$b$-edge. However now the center node must be external too. The extra two edges prohibit the center
nodes removal. Thus an $A$-hyperedge with \emph{three} incident nodes would replace the digram. Note
that, in this example, no compression would be achieved, because the start graph still contains all
original nodes, and because hyperedges are more expensive than ordinary ones. 
%It is however possible to
%construct graphs where non-compressing replacements are necessary to enable later replacements that
%do compress the graph.
%
%However, it is not always possible to use simple edges to represent digrams. Consider the graph in
%Figure~\ref{fig:intro_rank3_example}. Here, no matter which pair of connected edges is chosen, all
%three incident nodes are also incident to at least one edge that is not part of the chosen pair.
%Thus, if we want to represent the edge pair using a nonterminal, we can not remove one of the nodes
%as before, as that would leave an edge without a node. Therefore, we need to have an edge attached to
%all three of these nodes -- a hyperedge.
%
%However, in general, simple edges are not sufficient. Consider the graph in
%Figure~\ref{fig:intro_rank3_example}, which is only a slight modification from the graph represented
%by the grammar in Figure~\ref{fig:intro_grammar_example}. In this graph, no pair of edges can be
%removed, without leaving a ``dangling edge'' behind. For this reason, our compressor introduces
%hyperedges in such cases. The grammar in Figure~\ref{fig:intro_hGrammar_example} is an example of
%such a grammar using hyperedges to represent the graph. Note the use of colors for the external
%nodes of the rule and also for the edges connecting the hyperedges to the nodes of the graph:
%They are used to unambiguously match up the nodes when deriving an edge. This also introduces the
%notation used for graphs in the rest of the paper.
\begin{figure*}[!t]
    \centering
    \subfloat[]{\input{figures/intro_grammar_example}\label{fig:intro_grammar_example}}\qquad
    \subfloat[]{\input{figures/intro_rank3_example}\label{fig:intro_rank3_example}}\qquad
    \subfloat[]{\input{figures/hypergraph_example}\label{fig:hypergraph_example}}\qquad
    \subfloat[]{\input{figures/intro_derivation_example}\label{fig:intro_derivation_example}}
%    \subfloat[]{\input{figures/intro_hGrammar_example}\label{fig:intro_hGrammar_example}}\qquad
    \caption{Examples of a graph grammar \protect\subref{fig:intro_grammar_example}, a full
    derivation of this grammar \protect\subref{fig:intro_derivation_example}, a graph incompressible
    with \graphrepair \protect\subref{fig:intro_rank3_example}, and a hypergraph
    \protect\subref{fig:hypergraph_example}.
%    
%    and a modification to the graph,
%    which makes it impossible to represent it without hyperedges with a grammar using only digrams
%    in its rules (\protect\subref{fig:intro_rank3_example}).
    % and a grammar using hyperedges to represent this
    %modified graph (\protect\subref{fig:intro_hGrammar_example}).
    }
    \label{fig:intro_example}
\end{figure*}

%We call the nodes of a digram incident with both hyperedges \emph{central nodes}. In the previous
%example, the digram has one central node: the one that is not external.
%The generalization of RePair to graphs poses new challenges,
%not present in the string and tree cases:
%Assume we want to count every occurrence of a digram $d$ centered around a node
%of degree $k$. There are $O(k^2)$ possible edge pairs, thus $O(n\cdot k^2)$
%many occurrences of $d$ can occur in a graph of $n$ nodes. 
%Additionally, even if we can determine a set of all possible occurrences, we actually need a maximum sized
%\emph{non-overlapping} subset, i.e., where no two occurrences share an edge. 
%
Let us now discuss some of the challenges that come up when generalizing RePair to graphs. In each
round of RePair we need to find a digram with a maximal number of \emph{non-overlapping} occurrences
(i.e., occurrences that have no edge in common). In the classical string and tree cases of RePair, maximal
non-overlapping occurrences of a digram can be found by simple greedy search. In the graph case,
this is no longer possible.
%
Determining such a subset is hard: it can be obtain from the full (overlapping) set of occurrences
by \emph{maximum matching}; the most efficient algorithms for the latter (such as
``Blossom'') require  $O(|V|^2|E|)$ time, which is infeasible for large graphs.
Furthermore, this is just the time required to find such a list for one digram.
%
As seen in Figure~\ref{fig:all_digrams}, even for unlabeled, undirected graphs (without hyperedges)
there are already eight different digrams to be considered. To address these challenges,
%
%Even if we
%only consider unlabeled, undirected edges however, there already are eight different digrams to be
%considered (see Figure~\ref{fig:all_digrams}).
%\begin{figure}[!t]
%    \centering
%    \input{figures/all_digrams}
%\vspace*{-4mm}
%    \caption{Every possible digram using two unlabeled, undirected edges.}
%    \label{fig:all_digrams}
%\end{figure}
%To solve these problems,
we apply a greedy approximation. We
follow some given fixed order \ord of nodes. For every node $u$ of degree $k$, we count the
occurrences of $d$ centered around $u$, in a way that only $O(k)$ possible digram occurrences are
considered. 
The chosen node order can significantly affect the compression ratios.
%
%The node order \ord heavily influences the compression behavior. Consider the graph in
%Figure~\ref{fig:counting_example}. We want to find the non-overlapping occurrences of the digram in
%Figure~\ref{fig:counting_example_digram}. Note the nodes filled in black: they are called \emph{external nodes}
%and indicate where nodes of a production are merged with nodes incident with a nonterminal edge.
%Essentially this means here that every node in an occurrence needs to be incident with edges
%\emph{other} than the two edges of the occurrence. Figure~\ref{fig:counting_example_center} shows
%the non-overlapping occurrences found if we start in the central node of the graph. Using the DFS-type order
%given by the numbers in Figure~\ref{fig:counting_example_dfs}, three occurrences are determined.
%Using the ``jumping'' order in Figure~\ref{fig:counting_example_opt}, a maximum set of four
%non-overlapping occurrences is found. 
%Note that for strings and trees, maximum sets of non-overlapping occurrences can be
%obtained by simple orders (namely, left-to-right and post order).
%
%
%It should be noted that a different digram would be chosen for this graph
%by our algorithm, the one shown on the right of Figure~\ref{fig:grammar_example}.
%Here the two colored nodes are the external nodes. The original graph in
%Figure~\ref{fig:counting_example} can be obtained by replacing every $A$-labeled hyperedge
%in the left graph of Figure~\ref{fig:grammar_example} by the digram,
%while merging the colored nodes according to the colors of the hyperedge.
%(The node numbers in the figure will be important later).
%
%The grammar formalism we use is well-studied and known as context-free 
%hyperedge replacement (HR) grammars, see~\cite{Engelfriet:1997:CGG:267871.267874}.
The main contributions of the paper are:
\begin{enumerate}
    \item a generalization of RePair to graphs (\graphrepair),
    \item an extensive experimental evaluation of an implementation of \graphrepair, and
    \item a linear-time algorithm for $(s,t)$-reachability over grammar-compressed graphs.
\end{enumerate}
The experimental results are that
\graphrepair improves over state-of-the-art compressors for RDF graphs
and for version graphs (unions of similar graphs). 
%For some network graphs we observe
%good improvements.
We found that one indicator of compression
performance by our method is the number of equivalence classes of our particular node order
(which is a generalization of the node degree order).



==> matching.tex <==
\section{Matching}
\label{sec:matching-algorithms}
In this section we present a collection of algorithms matching a word
$w$ against $e$. First, we present an algorithm for arbitrary
deterministic regular expressions that uses the constructions from
Section~\ref{sec:testing-determinism} and lowest colored ancestor
queries to achieve expected time complexity
$O(|e|+|w|\log\log |e|)$. Next, we present a matching algorithm for
$k$-occurrence regular expressions in time $O(|e|+k|w|)$, which is
linear if $k$ is a constant. The most intricate matching algorithm
that we present in this paper is the path-decomposition algorithm.
It works in time $O(|e|+c_e|w|)$, where $c_e$ is the maximal depth of
alternating union and concatenation operators in $e$.
The three algorithms
above perform matching by providing a \emph{transition simulation
  procedure}: given a position $p$ and a symbol $a$ return the
position $q$ labeled $a$ that follows $p$, or $\nil$ if no such
position exists. If $e=(\#e')\$$, matching a word $w$ against $e'$ is
straightforward: begin with position $\#$, use the
transition simulation procedure iteratively on subsequent symbols of
$w$, and finally test if the position obtained after processing the
last symbol of $w$ is followed by $\$$.


The algorithms above allow to match multiple input words
$w_1,\ldots,w_N$ against one regular expression $e$: the corresponding
running times are obtained by replacing the factor $|w|$ by
$|w_1|+\ldots+|w_N|$. We also present an algorithm that 
runs in time $O(|e|+|w_1|+\ldots+|w_N|)$ for 
star-free deterministic regular expressions $e$, a setting in which
none of the previously mentioned algorithms guarantee linear
complexity.

In the reminder of this section, we fix a deterministic regular
expression $e$, and when talking about positions and nodes, we
implicitly mean positions and nodes of $e$.


\subsection{Lowest Colored Ancestor Algorithm}
\label{sec:lowest-color-ancest}
Our previous construction that tests determinism in linear time, 
provides an efficient procedure for transition simulation. 
Recall that we color
the parent of any $\isrootfirst$-node $n$ with the labels of the
positions that belong to $\First(n)$. By
Lemma~\ref{lem:info-is-in-color-ancestor}, given a position $p$ and a
symbol $a$ the $a$-labeled position $q$ that follows $p$ is one of:
$\Witness(n,a)$, $\Annotate(n,a)$, and $\Next(n,a)$, where $n$ is the
lowest ancestor of $p$ with color $a$. We use the $\checkIfFollow{}$
test (Theorem~\ref{th-checkIfFollow}) to select the correct following
position $q$ among the three candidates. 
\begin{example}\rm
  \label{ex:5}
  Consider the expression in Figure~\ref{fig:sample-regexp}, position
  $p_3$, and the symbol $c$. The lowest ancestor of $p_3$ with color
  $c$ is $n_3$. Here, $\Witness(n_3,c)=p_5$, $\Next(n_3,c)=p_1$, and
  $\Annotate(n_3,c)=\nil$. Using $\checkIfFollow$ we find that it is
  $p_5$ that follows $p_3$. This ends the transition simulation
  procedure.
  Now, at position $p_5$ we read the next symbol $a$. The lowest
  ancestor of $p_5$ with color $a$ is again $n_3$. This time it is
  $\Annotate(n_3,a)=p_2$ that follows $p_5$.
\end{example}
The basic ingredient of this procedure is an efficient algorithm for
answering lowest colored ancestor queries. Recall
from~\cite{Muthu96,FaMu95} (our lowest colored ancestor is called
 ``nearest colored ancestor'' there), that given a tree $t$ with colors assigned
to its nodes (some nodes possibly having multiple colors), we can
preprocess $t$ in expected time $O(|t|+C)$, where $C$ is the total
number of color assignments, so that any lowest colored ancestor query
is answered in time $O(\log\log |t|)$. In this way, the transition
simulation is accomplished in time $O(\log\log |e|)$, which gives
us the following result.
\begin{theorem}\rm
  \label{thm:semi-linear-matching}
  For any deterministic regular expression $e$, after preprocessing in
  expected time $O(|e|)$, we can decide for any word $w$ whether
  $w\in L(e)$ in time $O(|w|\log\log |e|)$.
\end{theorem}

\subsection{Bounded Occurrence Algorithm}
\label{sec:k-occurr-regul}
A regular expressions $e$ is called {\em k-occurrence} (\mbox{$k$-\ORE}
for short) if each symbol $a\in\Sigma$ occurs at most $k$ times in
$e$. While every regular expression is $k$-\ORE for a sufficiently large $k$, 
Bex, Neven, Schwentick, and Vansummeren~\cite{BexTods10} report that the majority of 
regular expressions in real-life XML schemas are in fact
\mbox{$1$-\ORE}s. Given a position $p$ and a symbol $a$, to find the
following $a$-labeled position $q$ we only need to perform the
$\checkIfFollow{}$ test (Theorem~\ref{th-checkIfFollow}) on all
$a$-labeled positions in $e$, which are gathered into a designated
list during preprocessing of $e$. Thus, transition simulation
is performed in time $O(k)$, which proves the following result:
\begin{theorem}\label{thm:kore-linear-matching}\rm
  For any deterministic $k$-\ORE $e$, after preprocessing in time
  $O(|e|)$, we can decide for any word $w$ whether $w\in L(e)$ in time
  $O(k|w|)$.
\end{theorem}
We note that an analogous technique can be used to match a word $w$
against a non-deterministic \mbox{$k$-\ORE} $e$: we maintain a set $P$
of at most $k$ positions and when reading symbol $a$ we identify among
the $a$-labeled positions those that follow any of the positions in
$P$. Here, reading one symbol requires $O(k^2)$ time, and thus, the
matching can be done in time $O(k^2|w|)$ after $O(|e|)$ preprocessing.

\subsection{Path Decomposition Algorithm}
\label{sec:path-decomp-algor}

Next, we describe an algorithm for matching a word $w$ against a
regular expression $e$ in time $O(|e|+c_e|w|)$, where $c_e$ is the
maximal depth of alternating union and concatenation operators in $e$
(as mentioned at the end of the Introduction, 
$c_e$ is bounded by $4$ in real-life \DTDs~\cite{gri10,GrijzenhoutM11}).
First, we define the function $\hf(n,a)$ that for a node $n$ and a
symbol $a$ returns the unique $a$-labeled position in $\First(n)$ and
$\nil$ if it does not exist. Queries of the form $\hf(n,a)$ can be
answered in constant time after preprocessing in time $O(|e|)$, but
since $\hf$ is not used in the final algorithm, we omit the
implementation details.


\paragraph{Climbing Algorithm.}
We first present a simple transition simulation procedure that uses
$\hf$, and later improve it to obtain the desired evaluation
algorithm. Given a position $p$ and a symbol $a$, it suffices to find
an ancestor $n$ of $p$ such that $q=\hf(\Rchild(n),a)$ follows $p$
(tested with $\checkIfFollow{}$). If such ancestor does not exists,
then $p$ has no $a$-labeled following position. The soundness of this
procedure follows from that of $\checkIfFollow$ and the completeness
from Lemma~\ref{lem:prfirst-is-on-path}. A na\"ive implementation
seeks the ancestor in question by climbing up the parse tree starting
from $p$, which yields $O(\depth(e))$ time per transition simulation
and overall $O(|e|+\depth(e)\cdot|w|)$ time for matching.


\paragraph{Path Decomposition.}
Our algorithm speeds up climbing the path using jumps that follow
precomputed pointers. The precomputed pointers lead to nodes where we
store an aggregation of the values of $\hf$ for several nodes skipped
during the jump. The pointers are defined using the notion of path
decomposition of the parse tree.

Recall that a \emph{path decomposition} of a tree is a set of
pairwise disjoint paths covering all nodes of the tree, and here, a
path means a sequence of nodes $n_1,\ldots,n_k$ such that $n_i$ is the
parent of $n_{i+1}$. Note that a path decomposition of a tree can be
specified by the set of the top-most nodes of the paths, 
which is how we define the path decomposition of $e$. 
A node $y$ of $e$ is the \emph{top-most node} of a
path if it is the root of $e$, or
satisfies one of the following conditions:
\begin{enumerate}
\item[(i)] $\isrootlast(y)$,
\item[(ii)] $\isrootfirst(y)$,
\item[(iii)] $y$ is the nullable right child of its parent, or
\item[(iv)] $y$ is the right child of a $+$-labeled node.
\end{enumerate}
For a position $p$ we define $\topNode(p)$ as the
top-most node of the path of the left sibling of $\prfirst(p)$. 
\begin{example}\rm
Consider the regular expression presented in
Figure~\ref{fig:path-decomp} together with its path decomposition.  
For this expression $c_e=4$ because there are at most
$4$ alternations of union and concatenation operators on any path of
the expression, and in particular, it is $4$ on the path from
$p_1$ to the root node. Note that $\topNode(p_1)=n_3$ and
$\topNode(p_2)=n_1$. 
\end{example}
\begin{figure}[bht]
\begin{center}
  % \definecolor{mycols}{RGB}{38,144,255}
  % \definecolor{mycols}{RGB}{180,124,70}
% \definecolor{Dandelion}{rgb}{.94,.88,.19}
  \colorlet{mycols}{Dandelion!80!white} %% 2
  \pgfdeclareverticalshading{myshadP}{100bp}
  {color(0bp)=(mycols!20!white); 
    color(50bp)=(mycols!8!white); 
    color(75bp)=(mycols!3!white); 
   color(100bp)=(mycols!0!white)}
 \begin{tikzpicture}[yscale=.72,xscale=1, 
   Srfirst/.style={
     circle, 
     inner sep=0.2mm,
     minimum size=5.5mm, 
     draw=LimeGreen, 
     very thick
   },
   Srlast/.style={
     circle, 
     inner sep=0.2mm,
     minimum size=5.5mm, 
     draw=orange, 
     ultra thick, 
     dotted
   },
   Scol/.style={
     above, 
     color=red
   },
   Sid/.style={
     right=5pt,
     font=\small, 
     color=Maroon
   },
   Sidpb/.style={
     below=-4pt,
     font=\small, 
     color=Navy
   },
   Sidpr/.style={
     above=4pt, 
     right=4pt,
     font=\small, 
     color=Navy},
   Svirtual/.style={
     color=black!60!white
   },
   % Spath/.style={blue!60!black, rounded corners, smooth cycle}
   Spath/.style={
     Grey!20!black, 
     draw=Dandelion!60!black, 
     thin,
     shading=myshadP,
     rounded corners,  
   },
   Swhite/.style={color=white,
   }
   ]
   \tikzset{every node/.style={circle, inner sep=.2mm, minimum size=6mm}}
   \tikzstyle{level 1}=[level distance=1.8cm, sibling distance=2.6cm]
   \tikzstyle{level 2}=[level distance=1.3cm, sibling distance=1.8cm]
   \tikzstyle{level 3}=[level distance=1.25cm, sibling distance=1.75cm]
   \tikzstyle{level 4}=[level distance=1.12cm, sibling distance=1.5cm]
   \tikzstyle{level 5}=[level distance=1.05cm, sibling distance=1.45cm]
   \tikzstyle{level 6}=[level distance=1cm, sibling distance=1.35cm]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	regular expression	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node[Swhite] at (0,0) (nr) {$\figbullet$}
  child { node[Swhite] (n1) {$\figbullet$}
    child { node[Swhite] (n11) {$\figbullet$}
      child { node[Swhite] (n111) {$?$}
	child { node[Swhite] (n1111) {$a$}}}
      child { node[Swhite] (n112) {$\figbullet$}
	child { node[Swhite] (n1121) {$\figbullet$}
	  child { node[Swhite] (n11211) {$?$}
	    child { node[Swhite] (n112111) {$b$}}}
	  child { node[Swhite] (n11212) {$+$}
	    child { node[Swhite] (n112121) {$c$}}
	    child { node[Swhite] (n112122) {$\figbullet$}
	      child { node[Swhite] (n1121221) {$+$}
		child { node[Swhite] (n11212211) {$+$}
		  child { node[Swhite] (n112122111) {$d$}}
		  child { node[Swhite] (n112122112) {$\figbullet$}
		    child { node[Swhite] (n1121221121) {$e$}}
		    child { node[Swhite] (n1121221122) {$?$}
		      child { node[Swhite] (n11212211221) {$a$}}}}}
		child { node[Swhite] (n11212212) {$f$}}}
	      child { node[Swhite] (n1121222) {$?$}
		child { node[Swhite] (n11212221) {$b$}}}}}}
	child { node[Swhite] (n1122) {$?$}
	      child { node[Swhite] (n11221) {$c$}}}}}
    child { node[Swhite] (n12) {$?$}
      child { node[Swhite] (n121) {$d$}}}}
  child { node[Swhite] (n2) {$+$}
    child { node[Swhite] (n21) {$e$}}
    child { node[Swhite] (n22) {$*$} 
      child { node[Swhite] (n221) {$+$}% possibly put a dot here then n2212 is Srfirst
	child { node[Swhite] (n2211) {$f$}}
	child { node[Swhite] (n2212) {$\fbullet$}
	  child { node[Swhite] (n22121) {$*$}
	    child { node[Swhite] (n221211) {$\fbullet$}
	      child { node[Swhite] (n2212111) {$g$}}
	      child { node[Swhite] (n2212112) {$*$}
		child { node[Swhite] (n22121121) {$\fbullet$}
		  child { node[Swhite] (n221211211) {$a$}}
		  child { node[Swhite] (n221211212) {$?$}
		    child { node[Swhite] (n2212112121) {$b$}}}}}}}
	  child { node[Swhite] (n22122) {$?$}
	    child { node[Swhite] (n221221) {$h$}
}}}}}}
;


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	the virtual nodes	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[Swhite,above left=20pt] at (nr) (nv1) {$\fbullet$};
\node[Swhite,above right=20pt] at (nv1) (nv2) {$\fbullet$};
\node[Swhite,below left=20pt] at (nv1) (nv3) {$\#$};
\node[Swhite,below right=20pt] at (nv2) (nv4) {$\$$};

\draw (nv1) edge (nv3) edge (nr)
(nv2)  edge (nv1) edge (nv4);

\draw[Spath] (nv2.west) -- (nv3.west) -- (nv3.south) -- (nv3.east) -- (nv2.east) --
(nv2.north) -- cycle;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	node[Swhite] identifiers	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[Sidpr,Swhite] at (n11212211221.south) {$p_1$};
\node[Sidpr,Swhite] at (n121.south) {$p_2$};
\node[Sidpb,Swhite] at (n2212111.south) {$p_3$};
\node[Sidpr,Swhite] at (n2212112121.south) {$p_4$};
\node[Sidpb,Swhite] at (n221221.south) {$p_5$};
\node[Sid,Swhite] at (nr) {$n_1$};
\node[Sid,Swhite] at (n112122) {$n_2$};
\node[Sid,Swhite] at (n112122112) {$n_3$};
\node[Sid,Swhite] at (n2) {\:$n_4$};
\node[Sid,Swhite] at (n2212) {$n_5$};
\node[Sid,Swhite] at (n221211212) {$n_6$};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	path decomposition	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[Spath] 
(nr.west)-- (n11.west) -- 
(n112.west) -- (n1121.west) -- (n11212.west) -- (n112121.west) --
(n112121.south) -- (n112121.east) -- (n11212.east) -- (n1121.east) -- 
(n112.east) -- (n11.east)-- (nr.east) -- (nr.north) -- cycle;

\draw[Spath] 
(n112122.west)-- (n112122111.west) -- (n112122111.south) -- (n112122111.east)
-- (n112122.east) -- (n112122.north) -- cycle;

\draw[Spath] 
(n22.north west) -- ($(n221.west)+(.06,0)$) -- (n2211.west) -- (n2211.south) -- (n2211.east) 
--  ($(n221.south east)+(0,0.1)$) -- (n22.north east) -- cycle;

\draw[Spath] 
 (n2212.west) -- ($(n22121.west)+(.06,.1)$) 
-- ($(n221211.west)+(.06,0)$) -- (n2212111.west) -- (n2212111.south) -- (n2212111.east)
-- ($(n221211.east)+(-0.06,-.14)$) -- ($(n22121.east)+(-0.06,-0.06)$) -- (n2212.east) --  (n2212.north) -- (n2212.west);


\draw[Spath] 
(n2212112.north west) -- ($(n22121121.west)+(.06,0)$) -- 
(n221211211.west)  -- (n221211211.south) -- (n221211211.east) -- 
($(n22121121.south east)+(0,.1)$) -- (n2212112.north east) -- cycle;

\draw[Spath] 
(n112122112.west) -- (n1121221121.west) -- (n1121221121.south) -- 
(n1121221121.east) -- (n112122112.east) -- (n112122112.north) -- cycle;

\draw[Spath] 
(n2.west) -- (n21.west) -- (n21.south) -- 
(n21.east) -- (n2.east) -- (n2.north) -- cycle;


%%%%%%%%%%%%%%%%%%
% vertical paths %
%%%%%%%%%%%%%%%%%%
\draw[Spath] 
(n111.north west) -- (n1111.south west) -- 
(n1111.south east) -- (n111.north east) -- cycle;

\draw[Spath] 
(n11211.north west) -- (n112111.south west) -- 
(n112111.south east) -- (n11211.north east) -- cycle;

\draw[Spath] 
(n12.north west) -- (n121.south west) -- 
(n121.south east) -- (n12.north east) -- cycle;

\draw[Spath] 
(n1122.north west) -- (n11221.south west) -- 
(n11221.south east) -- (n1122.north east) -- cycle;

\draw[Spath] 
(n1121222.north west) -- (n11212221.south west) -- 
(n11212221.south east) -- (n1121222.north east) -- cycle;

\draw[Spath] 
(n1121221122.north west) -- (n11212211221.south west) -- 
(n11212211221.south east) -- (n1121221122.north east) -- cycle;

\draw[Spath] 
(n22122.north west) -- (n221221.south west) -- 
(n221221.south east) -- (n22122.north east) -- cycle;

\draw[Spath] 
(n221211212.north west) -- (n2212112121.south west) -- 
(n2212112121.south east) -- (n221211212.north east) -- cycle;

%%%%%%%%%%%%%%%%%
% single node 	%
%%%%%%%%%%%%%%%%%
\draw[Spath] 
(n11212212.north west) -- (n11212212.south west) -- 
(n11212212.south east) -- (n11212212.north east) -- cycle;



%%%%%%%%%%%%%%%%%
% Legend        %
%%%%%%%%%%%%%%%%%
\node[Srfirst] at (2.4,2) (nrf) {\small $n$};
\node[right] at (nrf.east) {\small: $\isrootfirst(n)$};
\node[Srlast] at (2.4,1) (nrf) {\small $n$};
\node[right] at (nrf.east) {\small: $\isrootlast(n)$};
\node[] at (2.4,0) (nrl1) {$x$};
\node[] at (nrl1)[below=-3pt](nrl2) {};
\path [Spath] (nrl1.north west) -- (nrl2.south west)  -- 
(nrl2.south east) -- (nrl1.north east) -- cycle;
\node[right] at (nrl1.east)[yshift=-0.8mm] {\small: 
%\parbox[t]{2.5cm}{
path of the decomposition
%}
};

\draw[Silver,thin] (1.9,2.6) -- (7.2,2.6) -- (7.2,-.8) --  (1.9,-.8) -- cycle;

\node[Srfirst] at (0,0) (nr) {$\figbullet$}
  child { node (n1) {$\figbullet$}
    child { node (n11) {$\figbullet$}
      child { node[Srlast] (n111) {$?$}
	child { node (n1111) {$a$}}}
      child { node (n112) {$\figbullet$}
	child { node (n1121) {$\figbullet$}
	  child { node[Srlast] (n11211) {$?$}
	    child { node (n112111) {$b$}}}
	  child { node (n11212) {$+$}
	    child { node (n112121) {$c$}}
	    child { node (n112122) {$\figbullet$}
	      child { node (n1121221) {$+$}
		child { node (n11212211) {$+$}
		  child { node (n112122111) {$d$}}
		  child { node (n112122112) {$\figbullet$}
		    child { node (n1121221121) {$e$}}
		    child { node[Srfirst] (n1121221122) {$?$}
		      child { node (n11212211221) {$a$}}}}}
		child { node (n11212212) {$f$}}}
	      child { node[Srfirst] (n1121222) {$?$}
		child { node (n11212221) {$b$}}}}}}
	child { node[Srfirst] (n1122) {$?$}
	      child { node (n11221) {$c$}}}}}
    child { node[Srfirst] (n12) {$?$}
      child { node (n121) {$d$}}}}
  child { node[Srfirst] (n2) {$+$}
    child { node (n21) {$e$}}
    child { node (n22) {$*$} 
      child { node (n221) {$+$}% possibly put a dot here then n2212 is Srfirst
	child { node (n2211) {$f$}}
	child { node (n2212) {$\fbullet$}
	  child { node (n22121) {$*$}
	    child { node (n221211) {$\fbullet$}
	      child { node (n2212111) {$g$}}
	      child { node[Srfirst] (n2212112) {$*$}
		child { node (n22121121) {$\fbullet$}
		  child { node (n221211211) {$a$}}
		  child { node[Srfirst] (n221211212) {$?$}
		    child { node (n2212112121) {$b$}}}}}}}
	  child { node (n22122) {$?$}
	    child { node (n221221) {$h$}
}}}}}}
;


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	the virtual nodes	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[Svirtual,above left=20pt] at (nr) (nv1) {$\fbullet$};
\node[Svirtual,above right=20pt] at (nv1) (nv2) {$\fbullet$};
\node[Svirtual,below left=20pt] at (nv1) (nv3) {$\#$};
\node[Svirtual,below right=20pt] at (nv2) (nv4) {$\$$};

\draw (nv1) edge[Svirtual] (nv3) edge[Svirtual] (nr)
(nv2)  edge[Svirtual] (nv1) edge[Svirtual] (nv4);


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%	node identifiers	%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[Sidpr] at (n11212211221.south) {$p_1$};
\node[Sidpr] at (n121.south) {$p_2$};
\node[Sidpb] at (n2212111.south) {$p_3$};
\node[Sidpr] at (n2212112121.south) {$p_4$};
\node[Sidpb] at (n221221.south) {$p_5$};
\node[Sid] at (nr) {$n_1$};
\node[Sid] at (n112122) {$n_2$};
\node[Sid] at (n112122112) {$n_3$};
\node[Sid] at (n2) {\:$n_4$};
\node[Sid] at (n2212) {$n_5$};
\node[Sid] at (n221211212) {$n_6$};
\end{tikzpicture}
\end{center}
\caption{Path decomposition.}\label{fig:path-decomp}
\end{figure}

% \begin{example}
%   \label{ex:1}
% \end{example}

We now define the function $h$ which is similar to $\hf$ but
defined for top-most nodes only: $h(n,a)$ points to the $a$-labeled
position $p$ with $n=\topNode(p)$, i.e., we assign
$h(\topNode(p),\Lab(p))=p$ for every position $p$. For instance, in
the expression in Figure~\ref{fig:path-decomp}, $h(n_3,a)=p_1$ and
$h(n_1,d)=p_2$. 

There exists a subtle connection between $h$ and $\hf$. If we consider a
top-most node $n$, then the values of $h$ assigned to $n$ can be
viewed as an aggregation of values of $\hf$ of several nodes
$n_1,\ldots,n_k$, which are gathered from around the path (but not
from the path). The decomposition of $e$ ensures that the aggregation
is collision-free, i.e., if $\hf(n_i,a)\neq\nil$ for some $i$, then
$\hf(n_j,a)=\nil$ for all $j\neq i$. Formally, we state this property
as follows.
\begin{lemma}\rm
  For any two different positions $p$ and $p'$, if
  $\topNode(p)=\topNode(p')$, then $p$ and $p'$ have different labels.
\end{lemma}
\begin{proof}
  Let $y$ denote the lowest node in the path of $\topNode(p)$ and let
  $p_0$ denote some position in $\Last(y)$. We show that $p$ follows
  $p_0$. By definition of $\topNode(p)$, the left sibling of
  $\prfirst(p)$ is on the path between $y$ and
  $\topNode(p)$. Therefore, $\prlast(p_0)=\prlast(y)$ is an ancestor
  of the left sibling of $\prfirst(p)$ because there is no
  $\isrootlast$-node on a path except for the top-most node of the
  path. Moreover, we observe that the parent of $\prfirst(p)$ is
  labeled with $\lbullet$. Thus, by Lemma~\ref{lem:caract-follow} we
  get $p\in\FOllow(p_0)$. Similarly, we show that
  $p'\in\FOllow(p_0)$. Because $e$ is deterministic, there cannot be
  two different positions with the same label in $\FOllow(p_0)$.
\end{proof}

\paragraph{Lazy Arrays.}
To store the values of $h$ we use \emph{lazy arrays}, which we
describe in detail next. This interesting data structure is known in
programmer's circles~\cite{LazyarrayRMN09,LazyarrayMS90}; its first mention is,
as far as we known, in Exercise~2.12 of~\cite{DBLP:books/aw/AhoHU74}.
The data structure provides the
functionality of an associative array with constant time
initialization, assignment, and lookup operations. 
The finite set of keys $K$ needs to be known prior to initialization of the data
structure. Furthermore, every key needs to be associated with a unique
element from a continuous fragment of natural numbers, and here for
simplicity, we assume that $K=\{1,\ldots,N\}$ for some $N\geq 1$.

A lazy array consists of an array $A$ that stores the values
associated with the keys, a counter $C$ of active keys having a value
assigned, and additionally two arrays $B$ and $F$ that store the set
of active keys. At initialization, $C$ is set to $0$ and
uninitialized memory of length $N$ is allocated for each of the arrays $A$, $F$, and $B$
(an operation assumed to work in $O(1)$ time). To \emph{assign} value $v$
to key $k$, we add $k$ to the set of active keys 
(if $k$ is not in that set already), and assign $A[k]=v$. 
To \emph{lookup} key $k$, we return $A[k]$ if $k$ is active and 
return $\nil$ otherwise.
To add a key $k$ to the set of active keys, we increment $C$, 
set $F[C]=k$, and set $B[k]=C$. In this way a key $k$ is active 
if and only if $1 \leq B[k] \leq C$ and $F[B[k]] = k$. 
Note that the first condition alone is insufficient to check
if a key $k$ is active because $B$ has been allocated with
uninitialized memory.


We found out that in practice, hash arrays offer compatible
functionality with superior performance while theoretically providing
only expected $O(1)$ time for the assignment and lookup operations. As
a side note, we point out that lazy arrays stand on their own merit
because they allow a constant time reset operation (by simply setting
$C=0$), unmatched by hash arrays (but not needed by our algorithm).

\paragraph{Preprocessing.}
We construct and fill the lazy-array $h$ in one bottom-up traversal of
$e$. In the same traversal we also compute an additional pointer
$\nexttop$ for every position and every top-most node of a path,
defined as follows. We set $\nexttop(n)$ to the lowest top-most node
$y$ of a path above $\Parent(n)$ that is either the root of $e$, or
satisfies one of the following
conditions:
\begin{enumerate}
\item[(1)] $\isrootlast(y)$
\item[(2)] $\isrootfirst(y)$
\item[(3)] there exists a non-nullable $\lbullet$-labeled ancestor of
  $n$ in the path of $y$.
\end{enumerate}
For instance, in the expression in Figure~\ref{fig:path-decomp}, it holds
$\nexttop(p_3)=n_5$, $\nexttop(p_4)=n_6$, and $\nexttop(p_5)=n_4$. We
point out that $\nexttop(n)$ is always the top-most node of some path,
and furthermore, $\nexttop(n)$ is a strict ancestor of $n$.

\paragraph{Transition Simulation.}
$\FindNext$ in 
Algorithm~3 follows $\nexttop$ pointers on the path from
$p$ to the node $\prlast(p)$ while attempting to find 
$a$-labeled follow positions stored in $h$ at the visited nodes.
\begin{alg}{Transition simulation.}
  \PROCEDURE $\FindNext$($p$\,:\,Position, $a$\,:\,$\Sigma$)\,:\,Position\\
  \LN \tab $x\gets p$\\
  \LN \tab \WHILE $\prlast(p)\neq x$\\
  \LN \tab \tab \IF $\checkIfFollow(h(x,a),p)$ \\
  \LN \tab \tab \tab \THEN \RETURN $h(x,a)$\\
  \LN \tab \tab $x\gets \nexttop(x)$ \\
  \LN \tab \IF $\checkIfFollow(h(x,a),p)$ \\
  \LN \tab \tab \THEN \RETURN $h(x,a)$\\
  \LN \tab $y\gets \prfirst(\Parent(x))$\\
  \LN \tab \IF $y$ is nullable\\ 
  \LN \tab \tab \THEN $q\gets h(\nexttop(y),a)$ \\
  \LN \tab \tab \ELSE $q\gets h(\Lchild(\Parent(y)),a)$\\
  \LN \tab \IF $\checkIfFollow(q,p)$\\
  \LN \tab \tab \THEN \RETURN $q$\\
  \LN \tab \tab \ELSE \RETURN $\nil$\\
  \END \PROCEDURE
\end{alg}
If this does not succeed, then $\FindNext$ 
checks in $\First(\Parent(\prlast(p)))$ (Lines~8--14)
to find follow positions.
This task 
would be easy to accomplish with $\hf$ through
$\hf(\Parent(\prlast(p)),a)$. Since we wish to use $h$ instead, we
need to locate the node $n$ such that $h(n,a)$ returns the position we
look for. The location of this node depends on whether or not the node
$y=\Parent(\prlast(p))$ is nullable. If $y$ is nullable, we 
perform a single $\nexttop$ jump from $y$ to reach $n$. Otherwise, $n$
is the left sibling of $y$. Finally, we remark that if
$\hf(\Parent(\prlast(p)),a)$ is not $\nil$, then $h(n,a)$ returns the
same node. 
% but the converse needs not be true: even if $q=h(n,a)$ is
% not $\nil$, $\hf(\Parent(\prlast(p)),a)$ might be $\nil$. Consequently, we
% verify in Line~12 that the node $q$ indeed follows $p$.
\begin{example}\rm
  \label{ex:3}
  Consider expression in Figure~\ref{fig:path-decomp}, position
  $p_1$, and symbol $d$. The computation of $\FindNext(p_1,d)$ follows
  the jump sequence: $p_1, \Parent(p_1), n_3, n_2, n_1$. At node
  $n_1$, $h(n_1,d)$ yields position $p_2$, and since $p_2$ follows
  $p_1$, the procedure returns $p_2$.
\end{example}
\paragraph{Correctness.}
To reason about iterations of the main loop of $\FindNext$, we
introduce this notation: $\nexttop^0(n) = n$, and
$\nexttop^{i+1}(n)=\nexttop(\nexttop^i(n))$ for $i\geq0$. Also, the
\emph{jump sequence} of $p$ is the sequence
\[
\nexttop^0(p),\nexttop^1(p),\ldots,\nexttop^K(p),
\]
 where $K$ is 
such that $\nexttop^K(p)=\prlast(p)$. We call $K$ the
\emph{length} of the jump sequence of $p$. We first show that the main
loop performs a sufficient number of $\nexttop$ jumps.
\begin{lemma}\label{lem:next-pos-is-in-topsegments}\rm
  Let $p$ be a position. For every position $q$ that follows $p$, either
  $\topNode(q)$ belongs to the jump sequence or $q$
  belongs to $\First(\Parent(\prlast(p)))$.
\end{lemma}
\begin{proof}
%  Let $q$ a position in $\FOllow(p)$. 
  By Lemma~\ref{lem:prfirst-is-on-path} $\topNode(q)$ is an ancestor
  of $p$ or the left sibling of a non-nullable $\isrootfirst$-ancestor
  of $p$. Furthermore, if $\prfirst(q)$ is nullable then $\topNode(q)$
  is the top of the path containing $\Parent(\prfirst(q))$.  From the
  definition of $\topNode$ and $\nexttop$, the jump sequence of $p$
  visits every $\isrootfirst$- and $\isrootlast$-ancestor of $p$, as
  well as every ancestor $y$ of $p$ such that $y$ is top-most node of
  a path and there exists some non-nullable $\lbullet$-labeled
  ancestor of $p$ on that path.

  We assume that $q\notin\First(\Parent(\prlast(p)))$, and show that
  in this case $\topNode(q)$ belongs to the jump sequence.  Under
  that assumption, a case analysis for Lemma~\ref{lem:caract-follow}
  shows that $\prfirst(q)$ is the right sibling of $\prlast(p)$, or
  satisfies 
\[
\prlast(p)\Anc \Parent(\prfirst(q))\Anc p.
\]  If
  $\prfirst(q)$ is the right sibling of $\prlast(p)$, then
  $\topNode(q)$ is equal to $\prlast(p)$ and is therefore visited by
  the jump sequence.  Otherwise,
  $\prlast(p)\Anc \Parent(\prfirst(q))$.  By
  Lemma~\ref{lem:prlast-above-implies-null}, $\prfirst(q)$ is
  nullable.  Consequently, its parent belongs to the path of
  $\topNode(q)$.  Furthermore, the left sibling of $\prfirst(q)$, and
  therefore its parent, are non-nullable.  It follows that the parent
  of $\prfirst(q)$ is a non-nullable $\lbullet$-labeled ancestor of
  $p$ that belongs to the path of $\topNode(q)$. Hence $\topNode(q)$ belongs to the jump sequence.
\end{proof}
We now show the correctness of $\FindNext$.
\begin{lemma}\label{lem:correctness-transition-simulation-plusfree}\rm
  For any position $p$ and any symbol $a$, the procedure
  $\FindNext(p,a)$ returns $q$ iff $q\in\FOllow(p)$ and $\Lab(q)=a$.
\end{lemma}
\begin{proof}
  The soundness of $\FindNext$ follows from the use of
  $\checkIfFollow$ prior to returning a position. 
  Reciprocally, let $q\in\FOllow(p)$ with $\Lab(q)=a$.
  Then according to Lemma~\ref{lem:next-pos-is-in-topsegments}
  $\FindNext$ returns $q$ at Lines~4 or~7 if $q$ does not belong to $\First(\Parent(\prlast(p)))$,
  and at Line~13 otherwise.
\end{proof}

\paragraph{Complexity}
We show that the amortized running time of the transition
simulation procedure in Algorithm~3, 
when matching a word $w$ against the deterministic
regular expression $e$, is proportional to $c_e$, the maximal depth of
alternating union and concatenation operators in $e$.

\begin{lemma}\label{lem:complexity-analysis-transition-simulation-plusfree}\rm
  Procedure $\FindNext(p,a)$ works in amortized time $O(c_e)$, when
  matching a word against a deterministic regular expression $e$.
\end{lemma}
\begin{proof}
  We use the potential $\pot$ of the data structure defined as a
  function of the current position:
  \[
  \pot(p)=\card{\{v\Anc p\setsep \isrootfirst(v)\}}.
  \]
  At the phantom position $\#$, the initial potential is set to zero.
  The potential is increased by at most one each time the
  transition simulation procedure is executed.
  Now, let $q$ be the position returned by $\FindNext(p,a)$, i.e., the
  $a$-labeled position that follows $p$ in $e$. We prove that
  $\FindNext(p,a)$ executes at most $2(\pot(q)-\pot(p))+c_e+O(1)$
  iterations of the loop ($\nexttop$ jumps) before returning $q$.

  By definition of $\topNode$, there are no $\isrootfirst$-nodes between
  $\prfirst(q)$ and $\topNode(q)$, hence 
  \begin{equation}\label{eq:potential-pos-at-most-one-plus-top}
    \pot(q)\leq \pot(\topNode(q))+1. 
  \end{equation}
  Let $K$ be the length of the jump sequence of $p$ and let
  $n_i=\nexttop^i(p)$ for $0\leq i \leq K$. 
  Now, from the sequence
  $n_0,\ldots,n_K$ we remove every node that is the non-nullable right
  child of a $+$-labeled node and obtain a subsequence
  $n_{i_0},n_{i_1},\dots,n_{i_{K'}}$.  
  We show that for every $1\leq j\leq K'-2$, one of $n_j$ or $n_{j+1}$ is a $\isrootfirst$ node.
  If $n_{i_j}$ is not an $\isrootfirst$ node then by definition of the sequence it is the nullable right child of some $\fbullet$-labelled node,
  which is therefore also nullable.
  Then $n_{i_{j+1}}$ is a $\isrootfirst$-node by definition of $\nexttop$.
  Hence, for every $0 \leq j\leq K'$,
  \[
  j\leq 2(\pot(n_{i_0})-\pot(n_{i_j}))+2.
  \]
  Thus, for every $0 \leq j\leq K$,
  \begin{equation}\label{eq:potential-topnode-wrt-iterations}
    j\leq 2(\pot(p)-\pot(n_j))+2+K-K'.
  \end{equation}
  Let $\ell$ be the natural number such that $n_{\ell}=\topNode(q)$.
  Combining equations~\eqref{eq:potential-pos-at-most-one-plus-top}
  and~\eqref{eq:potential-topnode-wrt-iterations}, as $c_e$ is an
  upper bound for $K-K'$, we obtain the result claimed before:
  \begin{equation}
    \ell\leq 2(\pot(p)-\pot(q))+4+c_e.
  \end{equation}
  From this result, establishing the amortized complexity is 
  straightforward. Given a word $w=a_1\cdots a_n$, let $p_1,\dots,p_n$ be
  the sequence of positions with $p_i=\FindNext(p_{i-1},a_i)$ for
  $1\leq i \leq n$ and $p_0=\#$. Then, the number of iterations through
  the loop of $\FindNext$ while matching $w$ against $e$ is at most:
  \begin{align*}
    &n(4+c_e)+2\sum_{i=1}^{n}(\pot(p_{i-1})-\pot(p_{i}))\\
    &=n(4+c_e)+2(\pot(p_{0})-\pot(p_n))\\
    &\leq n(4+c_e).
  \end{align*}
  This implies the amortized cost of $O(c_e)$, because each line
  of $\FindNext$ runs in constant time.
\end{proof}

Note that in the previous proof it suffices to take a smaller value of $c_e$, 
the maximum number of ancestors of a position of $e$ that are labeled with $+$, 
are non-nullable, and have a parent labeled with $\lbullet$.
Lemmas~\ref{lem:correctness-transition-simulation-plusfree} and~\ref{lem:complexity-analysis-transition-simulation-plusfree} thus respectively 
guarantee the correctness and analyze the complexity of our algorithm that 
simulates successive transitions. This proves the following result:
\begin{theorem}\rm
  \label{thm:plus-free-matching}
  For any deterministic regular expression $e$, after preprocessing in
  time $O(|e|)$, we can decide for any word $w$ whether $w\in L(e)$ in
  time $O(c_e|w|)$, where $c_e$ is the maximal depth of alternating union and
  concatenation operators in $e$.
\end{theorem}


\subsection{Star-Free Algorithm}
Finally, we present an algorithm that matches simultaneously several
words $w_1,\ldots,w_N$ against a star-free deterministic regular
expression $e$ (i.e., one that contains no star $*$). 
For a single word this is trivial: in a
star-free regular expression, $q\in\FOllow(p)$ implies that position
$q$ is after $p$ in the preorder traversal of $e$, and therefore, to
simulate a transition it suffices to run the $\checkIfFollow$ test on
subsequent positions until a match is found. In fact, the
$\checkIfFollow$ tests can be hard-coded into the traversal to avoid
lowest common ancestor queries.

The result is non-trivial when matching several words
$w_1,\ldots,w_N$. Also this time, the expression is traversed only
once and for every word $w_i$ we maintain the current index $d_i$, 
indicating the prefix of $w_i$ matched so far. The
matching is driven by the preorder traversal of $e$: with
every position visited in the traversal we update the indices
$d_1,\ldots,d_N$ accordingly. The update process is, however, not
straightforward and to perform it efficiently we use a variant of 
$a$-skeleta, constructed dynamically.

First, we define some terminology. We say that the word $w_i$ at index
$d_i$ \emph{expects} the symbol $a$ if the symbol of $w_i$ at index
$d_i+1$ is $a$. We also say that $w_i$ at $d_i$ \emph{reaches}
position $p$ if after simulating transitions on the corresponding
prefix of $w_i$ we arrive at $p$ (or more precisely, the Glushkov
automaton of $e$ reaches $p$ after reading the prefix of $w_i$). A
\emph{dynamic $a$-skeleton} $t_a$ is essentially a structure
containing a subset of positions closed under lowest common
ancestors. Additionally, with each position $p$ in $t_a$ we associate
a list of (pointers to) words such that if word $w_i$ is associated
with $p$, then the word $w_i$ at index $d_i$ reaches the position $p$
and expects the symbol $a$.

When processing a position $p$ labeled $a$, we remove from the dynamic
$a$-skeleton $t_a$ every position $q$ that is followed by $p$, update
indices of the words on the list associated with $q$, and insert $p$
to some dynamic $a$-skeleta accordingly. We illustrate the procedure
in the following example.
\begin{example}\rm
  \label{ex:2}
  We consider the deterministic regular expression
  \[
e=(\#(((a+ba)(c?))(d?b)))\$,
\] where $\#$ and $\$$ are two phantom
  positions that do not need to be matched. The expression $e$ has 8
  positions: $\#,p_1,\dots,p_6,\$$. We match against $e$ the words
  $w_1=bcdb$, $w_2=acdba$, $w_3=acb$, and $w_4=bada$.

  Initially, all indices are $d_1=d_2=d_3=d_4=0$. When describing
  dynamic $a$-skeleta, we write $\langle p,W\rangle$ to indicate that
  a position $p$ has an associated list of words
  $W$. Initially, $t_a=\langle\#,[w_2,w_3]\rangle$,
  $t_b=\langle\#,[w_1,w_4]\rangle$, and all other dynamic $a$-skeleta
  are empty.

  In the first step, we read the $a$-labeled position $p_1$. Because
  $p_1$ follows $\#$, we remove from $t_a$ the position
  $\langle\#,[w_2,w_3]\rangle$, increment $d_2$ and $d_3$, and insert
  $\langle p_1,[w_2,w_3]\rangle$ to $t_c$. 

  Next, we read the $b$-labeled position $p_2$. Because $p_2$ follows
  $\#$, we remove from $t_b$ the position
  $\langle\#,[w_1,w_4]\rangle$, increment $d_1$ and $d_4$, and insert
  $\langle p_2,[w_4]\rangle$ to $t_a$ and $\langle p_2,[w_1]\rangle$
  to $t_c$. Because we keep the dynamic $a$-skeleta closed under
  lowest common ancestors, $t_c$ becomes $\langle p_1,[w_2,w_3]\rangle
  + \langle p_2,[w_1]\rangle$, where $+$ is a binary node whose
  children are $p_1$ and $p_2$.

  At the position $p_3$ labeled with $a$, because $p_3$ follows $p_2$,
  we remove $\langle p_2,[w_4]\rangle$ from $t_a$, increment $d_4$ and
  add $\langle p_3,[w_4]\rangle$ to $t_d$. At the position $p_4$
  labeled with $c$, because $p_4$ follows $p_1$, we remove from $t_c$
  the position $\langle p_1,[w_2,w_3]\rangle$, increment $d_2$ and
  $d_3$, and insert $\langle p_4,[w_2]\rangle$ to $t_d$ and $\langle
  p_4,[w_3]\rangle$ to $t_b$. Although $p_2$ is not followed by $p_4$,
  we also remove $\langle p_2,[w_1]\rangle$ from $t_c$ and discard it
  because we observe that $p_2$ will not be followed by any of the
  subsequent positions. After this step, $t_b=\langle
  p_4,[w_3]\rangle$, $t_c$ is empty, and $t_d=\langle p_3,[w_4]\rangle
  \lbullet \langle p_4,[w_2]\rangle$.

  The next position $p_5$ is labeled with $d$ and follows both $p_3$
  and $p_4$. Therefore, we remove from $t_d$ both $\langle
  p_3,[w_4]\rangle$ and $\langle p_4,[w_2]\rangle$, increment $d_2$
  and $d_4$, and insert $\langle p_5,[w_4]\rangle$ to $t_a$ and
  $\langle p_5,[w_2]\rangle$ to $t_b$. This way, $t_b$ is $\langle
  p_4,[w_3]\rangle\lbullet\langle p_5,[w_2]\rangle$. 

  In the last step we move to the position $p_6$ labeled with
  $b$. Because $p_6$ follows both $p_4$ and $p_5$, we remove $\langle
  p_5,[w_2]\rangle$ and $\langle p_4,[w_3]\rangle$ from $t_b$ and
  increment $d_2$ and $d_3$. We insert $\langle p_6,[w_2]\rangle$ to
  $t_a$. Because $d_3=|w_3|$ and $\$$ follows $p_6$, $w_3$ matches
  $e$. Since there are no further positions to process, the words
  $w_1$, $w_2$, and $w_4$ do not match $d$.
\end{example}
Details on how to efficiently handle $a$-skeleta follow. We assume
that the positions $p_1,\dots,p_m$ of $e$ are given in the traversal
order of $e$ and that $e$ has been preprocessed for LCA
and $\Last$ queries. Every time we process a position
$\langle{}p,W\rangle$, the list $W$ is nonempty and we increment the
index of every word in $W$, which corresponds to consuming one symbol
of every word in $W$. 
%Therefore, processing the positions throughout
%the execution of the algorithm sums up to 
%$O(|w_1|+\ldots+|w_N|)$. 
By $|t_a|$ we denote the number of all nodes
that are inserted to $t_a$ throughout the execution of the matching
algorithm. Note that for every consumed symbol we add to $a$-skeleta
at most one position and at most one additional LCA node. Therefore,
the sum of $|t_a|$ over $a\in\Sigma$ is in $O(|w_1|+\dots+|w_N|)$. We
shall use this observation when characterizing the total time
necessary to identify, remove, and insert positions in the dynamic
$a$-skeleta.

With every dynamic $a$-skeleton $t_a$ we maintain the right-most
position $p_a$, i.e., the position most recently added to $t_a$. We
also provide a procedure $\findLCA(t_a,p_i)$ for localizing in $t_a$
the possible position of the lowest common ancestor $n_\LCA$ of $p_a$
and a new position $p_i$ which follows $p_a$ in the traversal of
$e$. Note that $n_\LCA$ needs not be present in $t_a$ and
$\findLCA(t_a,p_i)$ returns the top-most descendant of $n_\LCA$
present in $t_a$ (which may possibly be $n_\LCA$ itself if $t_a$
contains it). The procedure simply climbs the right-most path in $t_a$
until the desired node is found. Furthermore, our algorithm performs
calls to $\findLCA$ with subsequent positions in the traversal order,
i.e., if a call $\findLCA(t_a,p_i)$ is followed by a call
$\findLCA(t_a,p_j)$, then $i<j$. The procedure $\findLCA$ takes
advantage of this assumption by saving the result of the previous call
and beginning to climb the right-most path of $t_a$ from the saved
node (if no new nodes have been added in between). This way the
cumulative execution time of all $\findLCA$ calls with $t_a$ is
$O(|t_a|)$, which sums over $a\in\Sigma$ to $O(|w_1|+\dots+|w_N|)$.

The $\findLCA$ procedure is used to insert new positions as well as to
identify and to remove relevant positions from the dynamic
$a$-skeleta. Inserting $p_i$ into $t_a$ is straightforward: we find
the lowest common ancestor $n_\LCA$ of $n_a$ and $p_i$ in $e$, use
$\findLCA(t_a,p_i))$ to find if and where to insert $n_\LCA$ to $t_a$, and
then insert $p_i$. Identifying and retrieving positions in $t_a$ that
are followed by $p_i$ is based on Lemma~\ref{lem:caract-follow}. We
climb the path from $\findLCA(t_a,p_i)$ to
$n_i=\Parent(\prfirst(p_i))$ and at every $\lbullet$-labeled node $n$
we pick the subtree $t'$ rooted at the left child of $n$. In one
traversal of $t'$ we retrieve all of its Last-positions, because they
are followed by $p_i$, and remove all remaining nodes, because none of
the remaining positions is followed by any of the subsequent positions
$p_{j\geq i}$. Again, because the number of nodes traversed by the
procedure in $t_a$ is proportional to $|t_a|$, the overall time
necessary to insert and remove positions in all $a$-skeleta is
$O(|w_1|+\dots+|w_N|)$, which justifies the following theorem:
\begin{theorem}\label{th:many-words-star-free}\rm
  For any star-free deterministic regular expression $e$ and 
  words $w_1,\dots, w_N$, we can decide
  which words belong to $L(e)$ in time
  $O(|e|+|w_1|+\dots+|w_N|)$.
\end{theorem}

\section{Matching Strongly Deterministic Regular Expressions}

% N B  with different conventions we could afford to keep counters at 0 by default and only increment to 1 when entering the subexpression, because we consider that maximum value for iterations is at least 2 (otherwise use quesiton mark) and 
% because of strong determinism 

% We call a configuration reachable if there exist a sequence of configurations $(p_1,c_1)\dots,(p_n,c_n)$

% % A transition from $p$ to $q$ can only take place if it the corresponding counter operations are valid. 
% % Namely:
% % \begin{itemize}
% %  \item A counter is not reset before
% % \end{itemize}
% % Those counter operations are a reformulation of the transitions in the counter automata of Gelade et al.~\cite{GeladeGM12}.
% % As a consequence, 
% % \begin{lemma}[\cite{GeladeGM12}]
% % Let $e$ be a strongly deterministic regular expression. Then for every word $w$, there is at most one possible valuation that 
% % \end{lemma}
% % A valuation $c$ is called \emph{reachable} if there is a word $w$ such that 

Consider an expression $e$ with numerical occurrence indicators.
For each node $n$ of $e$ we define $\nextiter(n)$ as a pointer 
to the closest iterative node among the strict ancestors of $n$
(and to $\nil$ otherwise).
We now adapt our three matching algorithms from the previous section 
to support numeric occurrence indicators, using pointer $\nextiter$ to examine and update the counters in 
relevant iterative subexpressions. 
The main difficulty is to maintain the efficiency while additionally traversing the pointers $\nextiter$.
Our matching algorithms in presence of numeric occurrence indicators 
rely again on an algorithm that tests if a configuration can follow another one. 
% According to remark~\ref{rk:intermediate-pointers-are-max-counters}, $c(x)=\max(x)$ for every $s\Anc x\Anc n$, 
% so in particular $c(x)\geq2$ and $c(x)$ will be reset during this transition  if the next position $q'$
% satisfies one of $q'=q$ or $\LCA(p,q')\Anc x$. 
% If we order carefully the candidates considered for the next position, all pointers  $\nextiter$ followed before 
% obtaining the correct iterative expressions correspond to a reset operations, which provides us with an amortization argument.

Algorithm~\ref{alg:checkiffollow-numocc} presents a general procedure to check if some position 
follows another one, given a valuation $c$ and the lowest iterative ancestor of the current position for which $c(x)<\min(x)$. 
To simplify algorithms using this procedure, we require from the procedure that it also returns the iterative 
expression corresponding to the transition if any, and $\fbullet$ otherwise.
\begin{proposition}\label{prop:correctness-checkfollow-numocc}\rm
Let $y_{<\min}$ be the lowest $y\Anc p$ for which $c(y)<\min(y)$, and $y_{<\min}$ is $\nil$ if there is no such $y$. 
Then Algorithm~\ref{alg:checkiffollow-numocc} returns $\false $ on $(p,q,c,y_{<\min})$ if and only if there are no $s,c'$ such that $(q,c')\in\FOllow^{s}(p,c)$, 
returns $(\true,\fbullet)$ if and only if there exists $c'$ such that $(q,c')\in\FOllow^{\fbullet}(p,c)$, 
and otherwise returns $(\true,s)$ where $s$ is the lowest iterative expression such that $(q,c')\in\FOllow^{s}(p,c)$.
\end{proposition}
\begin{proof}
It is clear that the algorithm checks the characterization above.
\end{proof}

\begin{alg}{Checking a candidate position}\label{alg:checkiffollow-numocc}
  \PROCEDURE $\checkIfFollow$($p,q$\,:\,Positions, $c$\,:\,valuation, $y_{<\min}$)\,:{\small\,Bool$\times$ Iterative expr.}\\
  \LN \tab $n\gets \LCA(p,q)$\\
  \LN \tab \IF $y_{<\min}\neq \nil$ \AND $n\Anc y_{<\min}$ \THEN \RETURN $(\false,\nil)$\\
  \LN \tab \IF $\Lab(n)=\lbullet$ \AND  $\prlast(p)\Anc n$ \AND $\prfirst(q)\Anc n$ \THEN \RETURN $(\true,\fbullet)$\\
  \LN \tab $s\gets \nextiter(n)$\\
  \LN \tab \WHILE $s\neq \nil$ \AND $\prlast(p)\Anc s$ \AND $\prfirst(q)\Anc s$ \AND $\max(s)=c(s)$\\%no need to check that $s\not\Anc \Listhead(l)$ since $\max(s)=c(s)$
  \LN \tab \tab $s\gets\nextiter(s)$\\
  \LN \tab \IF $s=\nil$ \OR $\max(s)=c(s)$\\
  \LN \tab \tab    \THEN \RETURN $(\false,\nil)$\\
  \LN \tab \tab \ELSE \RETURN $(\true,s)$\\
  \END \PROCEDURE
\end{alg}

\paragraph{Stacks and Pointers.}
We store two stacks in addition to the counters. The first stack $\ListMin$ keeps 
a pointer to the counter of every ancestor $n$ of the current position such that $c(n)<\min(n)$. 
The second stack $\Listtwo$ keeps a pointer to 
every ancestor $n$ of the current position such that $c(n)\geq2$ 
(these are the counters that may be reset during the execution of the algorithm).
The stack operations in Algorithm~\ref{alg:transition-simulation-numocc} guarantee that both stacks are ordered by decreasing depth of the nodes, so that the deepest nodes come on top. 
During preprocessing, we also build for each node $n$ a 
pointer $\nextiter(n)$ toward the closest iterative node 
among the strict ancestors of $n$, and another pointer $\miniter(n)$ toward the lowest iterative node 
among the strict ancestors of $n$ such that $\min(n)\geq2$.



\subsection{Bounded Occurrence Expressions}\label{subsec:kore-matching-numocc}

Assume that $e$ is a $k$-\ORE. Again we gather for each letter $a$ 
all $a$-labeled positions into a designated list during preprocessing, 
following the preorder.
%
When reading letter $a$ from position $p$, 
we first reorder the list of $a$-labeled positions into $q_1\dots q_k$
such that $q$ comes before $q'$ when $\LCA(p,q')$ is a strict ancestor of $\LCA(p,q)$.
This reordering can clearly be obtained with $O(k)$ operations. 
We then use procedure $\FindNextPoskocc$ which relies on the procedure $\checkIfFollow$ to check 
successively the candidate
positions $q_i$, and then updates the counters using $\ListMin$ and $\Listtwo$.

\begin{alg}{Transition Simulation for $k$-\ORE}\label{alg:transition-simulation-numocc}
 \GLOBVAR $\ListMin,\Listtwo$\,:\, Stacks of iterative nodes,
  $c$\,:\,valuation\\
  \PROCEDURE $\FindNextPoskocc$($p,q_1,q_2\dots,q_k$\,:\,Positions, $a$\,:\,$\Sigma$)\,:\,Position\\
  \LN \tab $i\gets 0$; $b\gets\false$\\
  \LN \tab \WHILE $i< k$ \AND $b=\false$\\
  \LN \tab \tab $i\gets i+1$\\
  \LN \tab \tab $(b,x)\gets \checkIfFollow(p,q_i,c,\Stacktop(\ListMin))$\\
  \LN \tab \IF $b=\false$ \THEN  \RETURN $\false$\\
  \LN \tab \ELSE\\
  \LN \tab \tab UpdateCounters($p,q_i,x$)\\
  \LN \tab \tab \RETURN $q_i$\\[.5cm]
  \PROCEDURE UpdateCounters($p,q_i,x$):\\
  \LN \tab $L_1\gets $ empty stack\\
  \LN \tab $s\gets x$\\
  \LN \tab \WHILE $\Listtwo$ is not empty \AND $\Stacktop(\Listtwo)\not\Anc s$\\
  \LN \tab \tab $c(\Stacktop(\Listtwo))\gets 1$\\
  \LN \tab \tab $\Stackpop(\Listtwo)$\\
%   \LN \tab Add all iterative ancestors $s\Anc z\Anc q_i$ to $\ListMin$, by increasing depth\\
  \LN \tab \IF $x\neq\fbullet$ \\
  \LN \tab \THEN \\
  \LN \tab \tab $c(x)\gets c(x)+1$ \\
  \LN \tab \tab \IF $\Stacktop(\Listtwo)\neq x$\\
  \LN \tab \tab \tab \THEN $\Stackpush{x}{\Listtwo}$\\
  \LN \tab \tab \IF $c(x)=\min(x)$\\
  \LN \tab \tab \tab \THEN $\Stackpop(\ListMin)$\hspace{2cm}//removes $x$ from $\ListMin$\\
%
  \LN \tab \tikzmark{na}  $z\gets\miniter(q_i)$\\
  \LN \tab \WHILE $z\neq \nil$ \AND $z\not\Anc s$\\ 
  \LN \tab \tab $\Stackpush{z}{L_1}$\\
  \LN \tab \tab $z\gets\miniter(z)$\\
  \LN \tab \WHILE $L_1$ is not empty\\
  \LN \tab \tab $z\gets \Stackpop( L_1)$\\
  \LN \tab \tikzmark{nb} \tab $\Stackpush{z}{\ListMin}$\\[.1cm]
% 
  \END \PROCEDURE
\begin{tikzpicture}[overlay, remember picture]
\draw [decoration={brace,amplitude=0.5em},decorate, thick,black]
    let \p1=(na), \p2=(nb) in
    ({max(\x1,\x2)+7cm}, {\y1+0.8em}) -- node[right=0.6em] {updates $\ListMin$} ({max(\x1,\x2)+7cm}, {\y2});
\end{tikzpicture}
\end{alg}

The correctness of the algorithm is guaranteed by Proposition~\ref{prop:correctness-checkfollow-numocc}:
using Lemma~\ref{lem:matching-in-terms-of-following-config} we can show that the counters and the two stacks are correctly updated. 
More interesting is the complexity of the algorithm.
Given a valuation ${c}$ for the counters and a node $n$, 
we define the first potential of $n$ as $\pot_{c}(n)=\{x\Anc n\sep c(x)\geq2\}$.
The iterations of the while loop inside $\checkIfFollow$ visit distinct nodes for every 
candidate position $q_i$. 
More importantly, each visited node $n$ satisfies $c(n)=\max(n)\geq2$. 
As the candidates are ordered by ascending order of $\LCA(p,q_i)$, 
the counter of every node thus visited is reset in the subsequent loops (Line~12). Furthermore, at most one counter is incremented while simulating the transitions (Line~16).
Consequently, the overall complexity of the calls to procedure $\checkIfFollow$ is bounded by 
$C_1(k+\pot_{c}(p)-\pot_{c'}(q_i)+2)$ for some constant $C_1$, where $p$ and ${c}$ (resp. $q_i$ and ${c'}$) are the current state and valuation before 
(resp. after) simulating the transition.
Similarly, the number of operations for updating $\Listtwo$ (Lines~13,17,18) can be bounded by 
$C_2(\pot_{c}(p)-\pot_{c'}(q_i)+2)$ for some constant $C_2$. 

Let us define the second potential of a node $n$ as $\pot_{c}'(n)=\{x\Anc n\sep c(x)< \min(x)\}$.
We observe that when a node is inserted into $\ListMin$, its counter has value $1$ and its minimal value is at least $2$ so 
that it contributes to the second potential for all its descendants. Furthermore, the second potential can decrease by at most one 
during a transition simulation since procedure $\checkIfFollow$ guarantees that nodes contributing to the second potential 
of $p$ are above $\LCA(p,q_i)$, and even above $x$ if $x\neq\nil$.
Thus the number of operations for updating $\ListMin$ (Lines~21 to~27) can be bounded by 
$C_3(\pot_{c'}'(q_i)-\pot_{c}'(p)+2)$ for some constant $C_3$.

For a large enough constant $C$, this gives an overall complexity of $C(\pot_{c}(p)-\pot_{c'}(q_i)+\pot_{c'}'(q_i)-\pot_{c}'(p)+4)$
for the cost of one transition simulation. % 3 is enough: I used 2 above so that we do not get 0 in case the amount is -1 but we just needed 1+epsilon (epsilon>0)
 From this result, establishing the amortized complexity is 
  straightforward. Given a word $w=a_1\cdots a_n$, let $p_1,\dots,p_n$ be
  the sequence of positions with $p_i=\FindNextPoskocc(p_{i-1},a_i)$ and $c_1,\dots,c_n$ the corresponding valuations, 
  for $1\leq i \leq n$ and $p_0=\#$. The results before show that for a large enough constant $C$, the number of operations while matching $w$ against $e$ is at most:
  \begin{align*}
    &Ckn+4Cn+C\sum_{i=0}^{n-1}(\pot_{c_i}(p_i)-\pot_{c_{i+1}}(p_{i+1}))+
    C\sum_{i=0}^{n-1}(\pot_{c_{i+1}}'(p_{i+1})-\pot_{c_i}'(p_i))\\
    &=Ckn+4Cn+C(\pot_{c_0}(p_0)-\pot_{c_n}(p_n)+\pot_{c_n}'(p_n)-\pot_{c_0}'(p_0))\\
    &\leq Ckn+ 6Cn\in O(kn).
  \end{align*}
We have thus established that deterministic $k$-\ORE expressions can still be evaluated in linear time (for fixed $k$) even in presence of counters:
\begin{theorem}\rm
 For every strongly deterministic k-\ORE with numerical occurrence indicators, 
after preprocessing in time $O(|e|)$, we 
 can decide if $w\in L(e)$ in time $O(k|w|)$.
\end{theorem}

\subsection{Lowest Colored Ancestor}

Instead of reordering the list of $a$-labeled positions into $q_1\dots q_k$ prior to verifying 
the certificates, 
we can can traverse the $a$-colored ancestors of $p$ using lowest-colored ancestor queries in $O(\log \log |e|)$, and 
take advantage of pointers $\Annotate(n,a)$ and $\Witness(n,a)$  
to check these positions in the order specified in Section~\ref{subsec:kore-matching-numocc}, i.e.,
such that $q$ comes before $q'$ when $\LCA(p,q')$ is a strict ancestor of $\LCA(p,q)$. 
Lemma~\ref{lem:info-is-in-color-ancestor} does not carry over in presence of numeric occurrence indicators, 
but it is obvious that the next position $q_i$ is still among $\Annotate(n,a)$ or $\Witness(n,a)$ for some $a$-colored ancestor $n$ of $p$. 
To visit the $q_i$ in desired order, 
we can consider the candidates from $\bigcup_{n\Anc p\textrm{ with color $a$}} \{\Witness(n,a),\Annotate(n,a)\}$ 
by height of $n$. We compute in constant time lowest common ancestors of $p$ with
 $\Annotate(n,a)$ and $\Witness(n,a)$ in order to decide which of these two positions should be considered first.
 One proves easily that with this approach the evaluation of deterministic expressions with counters has cost $O(|w|\log \log |e|)$ after the preprocessing:
\begin{theorem}\rm
 For every strongly deterministic expression with counters, after preprocessing in expected time $O(|e|)$, we 
 can decide if $w\in L(e)$ in time $O(|w|\log \log |e|)$. 
\end{theorem}


\subsection{Path Decomposition}
Instead of resorting to lowest colored ancestor queries, 
we can use the path decomposition idea 
to enumerate the candidates that need to be checked. 
The path decomposition algorithm for standard expressions enumerates the candidates $q_i$ in increasing
order of $\Parent(\prfirst(q_i))$. To restore the proper order for our numeric indicators algorithms (namely,  $q$ comes before $q'$ when $\LCA(p,q')$ is a strict ancestor of $\LCA(p,q)$), we combine this enumeration with pointers $\Annotate(n,a)$ 
as for the lowest colored ancestor algorithm. 
We slightly alter the definition of the $\nexttop$ pointers
to preserve the property that all relevant ancestors are traversed by the jump sequence
(a property whose proof depends on Lemma~\ref{lem:prlast-above-implies-null} in the absence of numeric occurrence indicators). 
For every node $n$ such that  $n$ is not nullable and $n$ is a $\isrootfirst$-node,
$\nexttop(n)$ is redefined as the left sibling of $n$. 
The transition simulation procedure must then be modified accordingly, so that the jump sequence only concludes 
on node $n$ if the two following conditions are satisfied simultaneously: 
$\isrootlast(n)$ and $n\Anc p$.
We can easily prove that after those modifications all relevant candidates are visited.


\begin{theorem}\rm
  \label{thm:plus-free-matching-counting}
  For any deterministic expression $e$ with numeric occurrence indicators, after preprocessing in
  time $O(|e|)$, we can decide for any word $w$ whether $w\in L(e)$ in
  time $O(c_e|w|)$, where $c_e$ is the maximal depth of alternating union and
  concatenation operators in $e$.
\end{theorem}
\begin{proof}
 To prove the correctness we only need to show that 
 the jump sequence in $\FindNext(p_i,a)$ with the alterations described above 
 traverses $\topNode(q)$ for every $a$-colored ancestor $n$ of $p_i$ such that $\prlast(p_i)$ is a strict ancestor of $n$, 
 and every $q\in\{\Annotate(n,a),\Witness(n,a)\}$ such that $q\notin\First(\Parent(\prlast(p_i)))$.
 The only case that differs from the proof of Lemma~\ref{lem:next-pos-is-in-topsegments} is when $\prlast(p_i)\Anc \Parent(\prfirst(q_i))$.
 Then, if $\prfirst(q_i)$ is nullable the argument follows as in Lemma~\ref{lem:next-pos-is-in-topsegments}, but $\prfirst(q_i)$ may also 
 be non-nullable (and still be a candidate in our list). If $\prfirst(q_i)$ is non-nullable,
 then its left sibling is a $\isrootlast$ node, and therefore is visited by our modified jump sequence, which concludes our  proof.

 For the complexity analysis, we observe that some $\isrootfirst$ ancestor of $p_i$ 
is visited every three iterations, instead of two for the jump sequence analyzed in Lemma~\ref{lem:complexity-analysis-transition-simulation-plusfree}.
As a consequence, the total cost over all transition simulations remains $O(c_e|w|)$ since our ordering of the candidates guarantees 
the total cost of processing counters is in $O(|w|)$ .
 \end{proof}


% \begin{alg}{Simulating iterative transitions}
%   \PROCEDURE $\FindNextIter$($p$\,:\,Position, $q$\,:\,Position, $a$\,:\,$\Sigma$,
%   $c$\,:\,valuation)\,:\,Position\\
%   \LN \tab $x\gets \nextiter(p)$\\
%   \LN \tab \WHILE $x\neq \nil$\\
%   \LN \tab \tab \IF $\prlast(p)\not\Anc x$ \THEN \RETURN $\false$\\
%   \LN \tab \tab \IF $c(x)<\min(x)$ \\
%   \LN \tab \tab \tab \THEN \IF $\hf(x,a)\neq\nil$\\
%   \LN \tab \tab \tab \tab \THEN $c(x)\gets c(x)+1$; \RETURN $\hf(x,a)$\\
%   \LN \tab \tab \tab \tab \ELSE \RETURN $\false$\\
%   \LN \tab \tab \tab \ELSE \IF $c(x)<\max(x)$ \AND $\hf(x,a)\neq\nil$\\
%   \LN \tab \tab \tab \tab \THEN $c(x)\gets c(x)+1$; \RETURN $\hf(x,a)$\\
%   \LN \tab \tab \tab \ELSE $c(x)\gets 1$; $x\gets\nextiter(x)$\\
%   \END \PROCEDURE
% \end{alg}
% 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

